Weak Collocation Regression for Inferring Stochastic Dynamics with L\'{e}vy Noise

With the rapid increase of observational, experimental and simulated data for stochastic systems, tremendous efforts have been devoted to identifying governing laws underlying the evolution of these systems. Despite the broad applications of non-Gaussian fluctuations in numerous physical phenomena, the data-driven approaches to extracting stochastic dynamics with L\'{e}vy noise are relatively few. In this work, we propose a Weak Collocation Regression (WCR) to explicitly reveal unknown stochastic dynamical systems, i.e., the Stochastic Differential Equation (SDE) with both $\alpha$-stable L\'{e}vy noise and Gaussian noise, from discrete aggregate data. This method utilizes the evolution equation of the probability distribution function, i.e., the Fokker-Planck (FP) equation. With the weak form of the FP equation, the WCR constructs a linear system of unknown parameters where all integrals are evaluated by Monte Carlo method with the observations. Then, the unknown parameters are obtained by a sparse linear regression. For a SDE with L\'{e}vy noise, the corresponding FP equation is a partial integro-differential equation (PIDE), which contains nonlocal terms, and is difficult to deal with. The weak form can avoid complicated multiple integrals. Our approach can simultaneously distinguish mixed noise types, even in multi-dimensional problems. Numerical experiments demonstrate that our method is accurate and computationally efficient.

==> License.tex <==
MIT License

Copyright (c) 2020 George Kour

Permission is hereby granted, free of charge, to any person obtaining a copy
of this software and associated documentation files (the "Software"), to deal
in the Software without restriction, including without limitation the rights
to use, copy, modify, merge, publish, distribute, sublicense, and/or sell
copies of the Software, and to permit persons to whom the Software is
furnished to do so, subject to the following conditions:

The above copyright notice and this permission notice shall be included in all
copies or substantial portions of the Software.

THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN NO EVENT SHALL THE
AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER
LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM,
OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE
SOFTWARE.


==> bib.tex <==
\begin{thebibliography}{10}

\bibitem{aguilar2017non}
Jean-Philippe Aguilar, Cyril~G Coste, and Jan Korbel.
\newblock Non-gaussian analytic option pricing: A closed formula for the l{\'e}vy-stable model.
\newblock {\em Available at SSRN 2828673}, 2017.

\bibitem{applebaum2009levy}
David Applebaum.
\newblock {\em L{\'e}vy processes and stochastic calculus}.
\newblock Cambridge university press, 2009.

\bibitem{bhat2022drift}
Harish~S Bhat.
\newblock Drift identification for l\'{e}vy alpha-stable stochastic systems.
\newblock {\em arXiv e-prints}, pages arXiv--2212, 2022.

\bibitem{black1973pricing}
Fischer Black and Myron Scholes.
\newblock The pricing of options and corporate liabilities.
\newblock {\em Journal of political economy}, 81(3):637--654, 1973.

\bibitem{boninsegna2018sparse}
Lorenzo Boninsegna, Feliks N{\"u}ske, and Cecilia Clementi.
\newblock Sparse learning of stochastic dynamical equations.
\newblock {\em The Journal of chemical physics}, 148(24):241723, 2018.

\bibitem{bowles2015weak}
Malcolm Bowles and Martial Agueh.
\newblock Weak solutions to a fractional fokker--planck equation via splitting and wasserstein gradient flow.
\newblock {\em Applied Mathematics Letters}, 42:30--35, 2015.

\bibitem{brunton2016discovering}
Steven~L Brunton, Joshua~L Proctor, and J~Nathan Kutz.
\newblock Discovering governing equations from data by sparse identification of nonlinear dynamical systems.
\newblock {\em Proceedings of the national academy of sciences}, 113(15):3932--3937, 2016.

\bibitem{bucher2015efficient}
Christian Bucher and Mario Di~Paola.
\newblock Efficient solution of the first passage problem by path integration for normal and poissonian white noise.
\newblock {\em Probabilistic Engineering Mechanics}, 41:121--128, 2015.

\bibitem{burkardt2021unified}
John Burkardt, Yixuan Wu, and Yanzhi Zhang.
\newblock A unified meshfree pseudospectral method for solving both classical and fractional pdes.
\newblock {\em SIAM Journal on Scientific Computing}, 43(2):A1389--A1411, 2021.

\bibitem{chen2021solving}
Xiaoli Chen, Liu Yang, Jinqiao Duan, and George~Em Karniadakis.
\newblock Solving inverse stochastic problems from discrete particle observations using the fokker--planck equation and physics-informed neural networks.
\newblock {\em SIAM Journal on Scientific Computing}, 43(3):B811--B830, 2021.

\bibitem{dai2023nonparametric}
Min Dai, Jinqiao Duan, Jianyu Hu, and Xiangjun Wang.
\newblock Nonparametric inference of stochastic differential equations based on the relative entropy rate.
\newblock {\em Mathematical Methods in the Applied Sciences}, 46(2):2986--2996, 2023.

\bibitem{dai2020detecting}
Min Dai, Ting Gao, Yubin Lu, Yayun Zheng, and Jinqiao Duan.
\newblock Detecting the maximum likelihood transition path from data of stochastic dynamical systems.
\newblock {\em Chaos: An Interdisciplinary Journal of Nonlinear Science}, 30(11):113124, 2020.

\bibitem{du2022discovery}
Qiang Du, Yiqi Gu, Haizhao Yang, and Chao Zhou.
\newblock The discovery of dynamics via linear multistep methods and deep learning: Error estimation.
\newblock {\em SIAM Journal on Numerical Analysis}, 60(4):2014--2045, 2022.

\bibitem{duan2015introduction}
Jinqiao Duan.
\newblock {\em An introduction to stochastic dynamics}, volume~51.
\newblock Cambridge University Press, 2015.

\bibitem{emmer2004optimal}
Susanne Emmer and Claudia Kl{\"u}ppelberg.
\newblock Optimal portfolios when stock prices follow an exponential l{\'e}vy process.
\newblock {\em Finance and Stochastics}, 8(1):17--44, 2004.

\bibitem{fang2022end}
Cheng Fang, Yubin Lu, Ting Gao, and Jinqiao Duan.
\newblock An end-to-end deep learning approach for extracting stochastic dynamical systems with $\alpha$-stable l{\'e}vy noise.
\newblock {\em Chaos: An Interdisciplinary Journal of Nonlinear Science}, 32(6), 2022.

\bibitem{ganzburg2008polynomial}
Michael~I Ganzburg.
\newblock Polynomial interpolation, an l-function, and pointwise approximation of continuous functions.
\newblock {\em Journal of approximation theory}, 153(1):1--18, 2008.

\bibitem{gao2016dynamical}
Ting Gao, Jinqiao Duan, Xingye Kan, and Zhuan Cheng.
\newblock Dynamical inference for transitions in stochastic systems with $\alpha$-stable l{\'e}vy noise.
\newblock {\em Journal of Physics A: Mathematical and Theoretical}, 49(29):294002, 2016.

\bibitem{gao2016fokker}
Ting Gao, Jinqiao Duan, and Xiaofan Li.
\newblock Fokker--planck equations for stochastic dynamical systems with symmetric l{\'e}vy motions.
\newblock {\em Applied Mathematics and Computation}, 278:1--20, 2016.

\bibitem{garcia2017nonparametric}
Constantino~A Garcia, Abraham Otero, Paulo Felix, Jesus Presedo, and David~G Marquez.
\newblock Nonparametric estimation of stochastic differential equations with sparse gaussian processes.
\newblock {\em Physical Review E}, 96(2):022104, 2017.

\bibitem{guo2022monte}
Ling Guo, Hao Wu, Xiaochen Yu, and Tao Zhou.
\newblock Monte carlo fpinns: Deep learning method for forward and inverse problems involving high dimensional fractional partial differential equations.
\newblock {\em Computer Methods in Applied Mechanics and Engineering}, 400:115523, 2022.

\bibitem{hu2022revealing}
Pipi Hu, Wuyue Yang, Yi~Zhu, and Liu Hong.
\newblock Revealing hidden dynamics from time-series data by odenet.
\newblock {\em Journal of Computational Physics}, 461:111203, 2022.

\bibitem{iman2008atin}
Ronald~L Iman.
\newblock Latin hypercube sampling.
\newblock {\em Encyclopedia of quantitative risk analysis and assessment}, 3, 2008.

\bibitem{kong2020sde}
Lingkai Kong, Jimeng Sun, and Chao Zhang.
\newblock Sde-net: Equipping deep neural networks with uncertainty estimates.
\newblock In {\em 37th International Conference on Machine Learning, ICML 2020}, pages 5361--5371. International Machine Learning Society (IMLS), 2020.

\bibitem{kwasnicki2017ten}
Mateusz Kwa{\'s}nicki.
\newblock Ten equivalent definitions of the fractional laplace operator.
\newblock {\em Fractional Calculus and Applied Analysis}, 20(1):7--51, 2017.

\bibitem{Lemieux2009MonteCA}
Christiane Lemieux.
\newblock Monte carlo and quasi-monte carlo sampling.
\newblock 2009.

\bibitem{li2021data}
Yang Li and Jinqiao Duan.
\newblock A data-driven approach for discovering stochastic dynamical systems with non-gaussian l{\'e}vy noise.
\newblock {\em Physica D: Nonlinear Phenomena}, 417:132830, 2021.

\bibitem{li2022extracting}
Yang Li, Yubin Lu, Shengyuan Xu, and Jinqiao Duan.
\newblock Extracting stochastic dynamical systems with $\alpha$-stable l\'{e}vy noise from data.
\newblock {\em Journal of Statistical Mechanics: Theory and Experiment}, 2022(2):023405, 2022.

\bibitem{long2018pde}
Zichao Long, Yiping Lu, Xianzhong Ma, and Bin Dong.
\newblock Pde-net: Learning pdes from data.
\newblock In {\em International conference on machine learning}, pages 3208--3216. PMLR, 2018.

\bibitem{lu2024weak}
Liwei Lu, Zhijun Zeng, Yan Jiang, Yi~Zhu, and Pipi Hu.
\newblock Weak collocation regression method: fast reveal hidden stochastic dynamics from high-dimensional aggregate data.
\newblock {\em Journal of Computational Physics}, 502:112799, 2024.

\bibitem{ma2021learning}
Shaojun Ma, Shu Liu, Hongyuan Zha, and Haomin Zhou.
\newblock Learning stochastic behaviour from aggregate data.
\newblock In {\em International Conference on Machine Learning}, pages 7258--7267. PMLR, 2021.

\bibitem{mantegna1996turbulence}
Rosario~N Mantegna and H~Eugene Stanley.
\newblock Turbulence and financial markets.
\newblock {\em Nature}, 383(6601):587--588, 1996.

\bibitem{matacz2000financial}
Andrew Matacz.
\newblock Financial modeling and option theory with the truncated l{\'e}vy process.
\newblock {\em International Journal of Theoretical and Applied Finance}, 3(01):143--160, 2000.

\bibitem{McKay1992lhs}
Michael~D. McKay.
\newblock Latin hypercube sampling as a tool in uncertainty analysis of computer models.
\newblock In {\em Proceedings of the 24th Conference on Winter Simulation}, page 557–564, New York, NY, USA, 1992. Association for Computing Machinery.

\bibitem{messenger2022learning}
Daniel~A Messenger and David~M Bortz.
\newblock Learning mean-field equations from particle data using wsindy.
\newblock {\em Physica D: Nonlinear Phenomena}, 439:133406, 2022.

\bibitem{opper2019variational}
Manfred Opper.
\newblock Variational inference for stochastic differential equations.
\newblock {\em Annalen der Physik}, 531(3):1800233, 2019.

\bibitem{pang2019fpinns}
Guofei Pang, Lu~Lu, and George~Em Karniadakis.
\newblock fpinns: Fractional physics-informed neural networks.
\newblock {\em SIAM Journal on Scientific Computing}, 41(4):A2603--A2626, 2019.

\bibitem{picchini2014inference}
Umberto Picchini.
\newblock Inference for sde models via approximate bayesian computation.
\newblock {\em Journal of Computational and Graphical Statistics}, 23(4):1080--1100, 2014.

\bibitem{rajabzadeh2016robust}
Yalda Rajabzadeh, Amir~Hossein Rezaie, and Hamidreza Amindavar.
\newblock A robust nonparametric framework for reconstruction of stochastic differential equation models.
\newblock {\em Physica A: Statistical Mechanics and its Applications}, 450:294--304, 2016.

\bibitem{schertzer2001fractional}
Daniel Schertzer, Michele Larchev{\^e}que, Jinqiao Duan, VV~Yanovsky, and Shaun Lovejoy.
\newblock Fractional fokker--planck equation for nonlinear stochastic differential equations driven by non-gaussian l{\'e}vy stable noises.
\newblock {\em Journal of Mathematical Physics}, 42(1):200--212, 2001.

\bibitem{sun2017governing}
Xu~Sun, Xiaofan Li, and Yayun Zheng.
\newblock Governing equations for probability densities of marcus stochastic differential equations with l\'{e}vy noise.
\newblock {\em Stochastics and Dynamics}, 17(05):1750033, 2017.

\bibitem{wei2015well}
Jinlong Wei and Rongrong Tian.
\newblock Well-posedness for the fractional fokker-planck equations.
\newblock {\em Journal of Mathematical Physics}, 56(3):031502, 2015.

\bibitem{yang2020generative}
Liu Yang, Constantinos Daskalakis, and George~Em Karniadakis.
\newblock Generative ensemble-regression: learning stochastic dynamics from discrete particle ensemble observations.
\newblock 2020.

\bibitem{yanovsky2000levy}
VV~Yanovsky, AV~Chechkin, D~Schertzer, and AV~Tur.
\newblock L{\'e}vy anomalous diffusion and fractional fokker--planck equation.
\newblock {\em Physica A: Statistical Mechanics and its Applications}, 282(1-2):13--34, 2000.

\bibitem{yu2021onsagernet}
Haijun Yu, Xinyuan Tian, E~Weinan, and Qianxiao Li.
\newblock Onsagernet: Learning stable and interpretable dynamics using a generalized onsager principle.
\newblock {\em Physical Review Fluids}, 6(11):114402, 2021.

\bibitem{zan2020stochastic}
Wanrong Zan, Yong Xu, J{\"u}rgen Kurths, Aleksei~V Chechkin, and Ralf Metzler.
\newblock Stochastic dynamics driven by combined l{\'e}vy--gaussian noise: fractional fokker--planck--kolmogorov equation and solution.
\newblock {\em Journal of Physics A: Mathematical and Theoretical}, 53(38):385001, 2020.

\bibitem{zan2021first}
Wanrong Zan, Yong Xu, Ralf Metzler, and J{\"u}rgen Kurths.
\newblock First-passage problem for stochastic differential equations with combined parametric gaussian and l\'{e}vy white noises via path integral method.
\newblock {\em Journal of Computational Physics}, 435:110264, 2021.

\bibitem{zhao2022adaptive}
Zichen Zhao and Qianxiao Li.
\newblock Adaptive sampling methods for learning dynamical systems.
\newblock In {\em Mathematical and Scientific Machine Learning}, pages 335--350. PMLR, 2022.

\bibitem{zheng2020maximum}
Yayun Zheng, Fang Yang, Jinqiao Duan, Xu~Sun, Ling Fu, and J{\"u}rgen Kurths.
\newblock The maximum likelihood climate change for global warming under the influence of greenhouse effect and l{\'e}vy noise.
\newblock {\em Chaos: An Interdisciplinary Journal of Nonlinear Science}, 30(1):013132, 2020.

\end{thebibliography}

